Nuclear structure calculations for neutron-star crusts

The goal of this paper is to investigate properties of clusterized nuclear matter which is believed to be present in crusts of neutron stars at subnuclear densities. It is assumed that the whole system can be represented by the set of Wigner-Seitz cells, each containing a nucleus and an electron background under the condition of electroneutrality. The nuclear structure calculations are performed within the relativistic mean-field model with the NL3 parametrization. The first set of calculations is performed assuming the constant electron background. The evolution of neutron and proton density distributions was systematically studied along isotopic chains until very neutron-rich system beyond the neutron dripline. Then we have replaced the uniform electron background with the realistic electron distributions, obtained within the Thomas-Fermi approximation in a self-consistent way with the proton distributions. Finally, we have investigated the evolution of the $\beta$-stability valley as well as neutron and proton driplines with the electron density.

==> library.tex <==
@book{Haensel2007,
address = {New York, NY},
doi = {10.1007/978-0-387-47301-7},
editor = {Haensel, P. and Potekhin, A. Y. and Yakovlev, D. G.},
isbn = {978-0-387-33543-8},
publisher = {Springer New York},
series = {Astrophysics and Space Science Library},
title = {{Neutron Stars 1}},
url = {http://link.springer.com/10.1007/978-0-387-47301-7},
volume = {326},
year = {2007}
}
@incollection{Pethick1991,
address = {Dordrecht},
author = {Pethick, C. J. and Ravenhall, D. G.},
booktitle = {Neutron Stars: Theory and Observation},
doi = {10.1007/978-94-011-3536-8_1},
pages = {3--20},
publisher = {Springer Netherlands},
title = {{An Introduction to Matter at Subnuclear Densities}},
url = {http://link.springer.com/10.1007/978-94-011-3536-8{\_}1},
year = {1991}
}
@article{Baym1971,
author = {Baym, Gordon and Pethick, Christopher and Sutherland, Peter},
doi = {10.1086/151216},
issn = {0004-637X},
journal = {The Astrophysical Journal},
month = {dec},
pages = {299},
title = {{The Ground State of Matter at High Densities: Equation of State and Stellar Models}},
url = {http://adsabs.harvard.edu/doi/10.1086/151216},
volume = {170},
year = {1971}
}
@article{Gogelein2007,
author = {G{\"{o}}gelein, P. and M{\"{u}}ther, H.},
doi = {10.1103/PhysRevC.76.024312},
issn = {0556-2813},
journal = {Physical Review C},
month = {aug},
number = {2},
pages = {024312},
title = {{Nuclear matter in the crust of neutron stars}},
url = {https://link.aps.org/doi/10.1103/PhysRevC.76.024312},
volume = {76},
year = {2007}
}
@article{Sharma2015,
author = {Sharma, B. K. and Centelles, M. and Vi{\~{n}}as, X. and Baldo, M. and Burgio, G. F.},
doi = {10.1051/0004-6361/201526642},
issn = {0004-6361},
journal = {Astronomy {\&} Astrophysics},
month = {dec},
pages = {A103},
title = {{Unified equation of state for neutron stars on a microscopic basis}},
url = {http://www.aanda.org/10.1051/0004-6361/201526642},
volume = {584},
year = {2015}
}
@article{Jin2017,
author = {Jin, Shi and Bulgac, Aurel and Roche, Kenneth and Wlaz{\l}owski, Gabriel},
doi = {10.1103/PhysRevC.95.044302},
issn = {2469-9985},
journal = {Physical Review C},
month = {apr},
number = {4},
pages = {044302},
title = {{Coordinate-space solver for superfluid many-fermion systems with the shifted conjugate-orthogonal conjugate-gradient method}},
url = {http://link.aps.org/doi/10.1103/PhysRevC.95.044302},
volume = {95},
year = {2017}
}
@article{Pastore2011,
author = {Pastore, Alessandro and Baroni, Simone and Losa, Cristina},
doi = {10.1103/PhysRevC.84.065807},
issn = {0556-2813},
journal = {Physical Review C},
month = {dec},
number = {6},
pages = {065807},
title = {{Superfluid properties of the inner crust of neutron stars}},
url = {https://link.aps.org/doi/10.1103/PhysRevC.84.065807},
volume = {84},
year = {2011}
}
@article{Than2011,
author = {Than, Hoang Sy and Khan, E and {Van Giai}, Nguyen},
doi = {10.1088/0954-3899/38/2/025201},
issn = {0954-3899},
journal = {Journal of Physics G: Nuclear and Particle Physics},
month = {feb},
number = {2},
pages = {025201},
title = {{Wigner–Seitz cells in neutron star crust with finite-range interactions}},
url = {http://stacks.iop.org/0954-3899/38/i=2/a=025201?key=crossref.614a4c6063ffc2718cb35686c18a2649},
volume = {38},
year = {2011}
}
@article{Baldo2007,
author = {Baldo, M. and Saperstein, E. E. and Tolokonnikov, S. V.},
doi = {10.1140/epja/i2006-10356-5},
issn = {1434-6001},
journal = {The European Physical Journal A},
month = {apr},
number = {1},
pages = {97--108},
title = {{A realistic model of superfluidity in the neutron star inner crust}},
url = {http://link.springer.com/10.1140/epja/i2006-10356-5},
volume = {32},
year = {2007}
}
@article{Grill2011,
author = {Grill, F. and Margueron, J. and Sandulescu, N.},
doi = {10.1103/PhysRevC.84.065801},
issn = {0556-2813},
journal = {Physical Review C},
month = {dec},
number = {6},
pages = {065801},
title = {{Cluster structure of the inner crust of neutron stars in the Hartree-Fock-Bogoliubov approach}},
url = {https://link.aps.org/doi/10.1103/PhysRevC.84.065801},
volume = {84},
year = {2011}
}
@article{Lalazissis1997,
author = {Lalazissis, G. A. and K{\"{o}}nig, J. and Ring, P.},
doi = {10.1103/PhysRevC.55.540},
issn = {0556-2813},
journal = {Physical Review C},
month = {jan},
number = {1},
pages = {540--543},
title = {{New parametrization for the Lagrangian density of relativistic mean field theory}},
url = {https://link.aps.org/doi/10.1103/PhysRevC.55.540},
volume = {55},
year = {1997}
}
@article{Furusawa2017,
author = {Furusawa, Shun and Mishustin, Igor},
doi = {10.1103/PhysRevC.95.035802},
issn = {2469-9985},
journal = {Physical Review C},
month = {mar},
number = {3},
pages = {035802},
title = {{Self-consistent calculation of the nuclear composition in hot and dense stellar matter}},
url = {https://link.aps.org/doi/10.1103/PhysRevC.95.035802},
volume = {95},
year = {2017}
}
@article{Chamel2007,
author = {Chamel, N. and Naimi, S. and Khan, E. and Margueron, J.},
doi = {10.1103/PhysRevC.75.055806},
issn = {0556-2813},
journal = {Physical Review C},
month = {may},
number = {5},
pages = {055806},
title = {{Validity of the Wigner-Seitz approximation in neutron star crust}},
url = {https://link.aps.org/doi/10.1103/PhysRevC.75.055806},
volume = {75},
year = {2007}
}
@article{Bender2000,
author = {Bender, M. and Rutz, K. and Reinhard, P. -G. and Maruhn, J. A.},
doi = {10.1007/s10050-000-4504-z},
issn = {1434-6001},
journal = {The European Physical Journal A},
month = {jul},
number = {1},
pages = {59--75},
title = {{Pairing gaps from nuclear mean-fieldmo dels}},
url = {http://link.springer.com/10.1007/s10050-000-4504-z},
volume = {8},
year = {2000}
}
@article{Baldo2006,
author = {Baldo, M. and Saperstein, E.E. and Tolokonnikov, S.V.},
doi = {10.1016/j.nuclphysa.2006.07.003},
issn = {03759474},
journal = {Nuclear Physics A},
month = {sep},
number = {3-4},
pages = {235--244},
title = {{The role of the boundary conditions in the Wigner–Seitz approximation applied to the neutron star inner crust}},
url = {http://linkinghub.elsevier.com/retrieve/pii/S0375947406004143},
volume = {775},
year = {2006}
}
@book{Glendenning2000,
abstract = {White dwarfs, neutron stars, and (solar mass) black holes are the collapsed cores of stars which, near the ends of their luminous lives, have shed most of their mass in supernova explosions or other, less spectacular, instabilities. Here gravity crushes matter to realms that lie far beyond present empirical knowledge. This book explores the diverse forms that such compact stars can possibly take, as constrained by the laws of nature: the general principles of relativity and quantum mechanics, the properties of nuclear matter deduced from nuclei, and the asymptotic freedom of quarks at high density. The book is self contained. It reviews general relativity, essential aspects of nuclear and particle physics, and general features of white dwarfs, neutron stars and black holes; it includes background on such matters as stellar formation and evolution, the discovery of pulsars and associated phenomena, and the strange-matter hypothesis. The book develops a theory for the constitution of neutron stars and the more exotic Hyperon Stars, Hybrid Stars (containing a quark matter core surrounded by an intricate lattice of quark and hadronic matter) and Strange Stars and Dwarfs (composed of the three light quark flavors sheathed in a solid skin of heavy ions). This second edition has been revised throughout to clarify discussions and bring data up to date; it includes new figures, several new sections, and new chapters on Bose condensates in neutron stars and on phase transitions.},
author = {Glendenning, N K},
booktitle = {Compact stars nuclear physics particle physics and general relativity Norman K Glendenning New York Springer 2000 Astronomy and astrophysics library},
doi = {10.1016/0370-1573(94)90166-X},
isbn = {9780387989778},
issn = {03701573},
number = {4-6},
pages = {313--332},
title = {{Compact stars: nuclear physics, particle physics, and general relativity}},
url = {http://linkinghub.elsevier.com/retrieve/pii/037015739490166X},
volume = {242},
year = {2000}
}
@article{Negele1973,
abstract = {An extremely simple form for the energy density of a nuclear many-body system derived from the two-body nucleon-nucleon interaction is used to determine the ground state configuration of matter at sub-nuclear density. As the baryon density is increased, nuclei become progressively more neutron rich until neutrons eventually escape, yielding a Coulomb lattice of bound neutron and proton clusters surrounded by a dilute neutron gas. The clusters enlarge and the lattice constant decreases with increasing density, approaching a completely uniform state near nuclear density. ?? 1973.},
author = {Negele, J. W. and Vautherin, D.},
doi = {10.1016/0375-9474(73)90349-7},
issn = {03759474},
journal = {Nuclear Physics, Section A},
number = {2},
pages = {298--320},
title = {{Neutron star matter at sub-nuclear densities}},
volume = {207},
year = {1973}
}
@article{Lattimer1985,
abstract = {The thermodynamic properties of hot, dense matter are examined in the density range 10−5 fm−3 ⩽ n ⩽ 0.35 fm−3 and the temperature range 0 ⩽ T ⩽ 21 MeV, for fixed lepton fractions Yℓ = 0.4, 0.3 and 0.2 and for matter in $\beta$-equilibrium with no neutrinos. Three phases of the matter are considered: the nuclei phase is assumed to consist of Wigner-Seitz cells with central nuclei surrounded by a nucleon vapor containing also $\alpha$-particles; in the bubbles phase the cell contains a central spherical bubble of nucleon vapor surrounded by dense nuclear matter; the third phase is that of uniform nuclear matter. All are immersed in a sea of leptons (electrons and neutrinos) and photons. The nuclei and bubbles are described by a compressible liquid drop model which is self-consistent in the sense that all of the constituent properties — bulk, surface, Coulomb energies and other minor contributions — are calculated from the same nuclear effective hamiltonian, in this case the Skyrme 1' interaction. The temperature dependence of all of these energies is included, for bulk and surface energies by direct calculation, for the Coulomb energy by combining in a plausible way the usual electrostatic energy and the numerical results pertaining to a hot Coulomb plasma. Lattice contributions to the Coulomb energy are an essential ingredient, and lattice modifications to the nuclear translational energy are included. A term is constructed to allow also for the reduced density of excited states of light nuclei. All of these modifications incorporate necessary physical effects which modify significantly the matter properties in some regions.},
author = {Lattimer, J.M. and Pethick, C.J. and Ravenhall, D.G. and Lamb, D.Q.},
doi = {10.1016/0375-9474(85)90006-5},
issn = {03759474},
journal = {Nuclear Physics A},
month = {jan},
number = {3},
pages = {646--742},
title = {{Physical properties of hot, dense matter: The general case}},
url = {http://linkinghub.elsevier.com/retrieve/pii/0375947485900065},
volume = {432},
year = {1985}
}
@article{Ravenhall1983,
abstract = {$\backslash$nIt is found that just below nuclear saturation density more stable forms of dense matter exist than the near-spherical nuclei or bubbles customarily assumed. Because of the large effect of the Coulomb lattice energy, cylindrical and planar geometries can occur, both as nuclei and as bubbles. It is suggested that in order to approximate more complicated kinds of short-range order, the dimensionality should be regarded as a continuous variable ranging from d=3 (spheres) to d=1 (planes). The dependence of d on density is illustrated, and its dependence on nuclear models discussed.},
author = {Ravenhall, D. G. and Pethick, C. J. and Wilson, J. R.},
doi = {10.1103/PhysRevLett.50.2066},
issn = {00319007},
journal = {Physical Review Letters},
number = {26},
pages = {2066--2069},
title = {{Structure of matter below nuclear saturation density}},
volume = {50},
year = {1983}
}
@article{Mishustin2010,
abstract = {Due to a first-order phase transition, a compact star may have a discontinuous distribution of baryon as well as electric charge densities, as e.g. at the surface of a strange quark star. The induced separation of positive and negative charges may lead to generation of supercritical electric fields in the vicinity of such a discontinuity. We study this effect within a relativistic Thomas-Fermi approximation and demonstrate that the strength of the electric field depends strongly on the degree of sharpness of the surface. The influence of strong electric fields on the stability of compact stars is discussed. It is demonstrated that stable configurations appear only when the counter-pressure of degenerate fermions is taken into consideration.},
archivePrefix = {arXiv},
arxivId = {1002.2541},
author = {Mishustin, Igor N and Ebel, Claudio and Greiner, Walter},
doi = {10.1088/0954-3899/37/7/075201},
eprint = {1002.2541},
issn = {0954-3899},
journal = {Journal of Physics G: Nuclear and Particle Physics},
number = {7},
pages = {075201},
title = {{Strong electric fields induced on a sharp stellar boundary}},
url = {http://stacks.iop.org/0954-3899/37/i=7/a=075201?key=crossref.3f5b808e5796d0ffff573bd4c57a5dda},
volume = {37},
year = {2010}
}
@article{Ebel2015,
abstract = {We study the electrostatic properties of inhomogeneous nuclear matter which can be formed in the crusts of neutron stars or in supernova explosions. Such matter is represented by Wigner–Seitz cells of different geometries (spherical, cylindrical, cartesian), which contain nuclei, free neutrons and electrons under the conditions of electrical neutrality. Using the Thomas–Fermi approximation, we have solved the Poisson equation for the electrostatic potential and calculated the corresponding electron density distributions in individual cells. The calculations are done for different shapes and sizes of the cells and different average baryon densities. The electron-to-baryon fraction was fixed at 0.3. Using realistic electron distributions leads to a significant reduction in electrostatic energy and electron chemical potential.},
author = {Ebel, Claudio and Mishustin, Igor and Greiner, Walter},
doi = {10.1088/0954-3899/42/10/105201},
issn = {0954-3899},
journal = {Journal of Physics G: Nuclear and Particle Physics},
month = {oct},
number = {10},
pages = {105201},
title = {{Realistic electrostatic potentials in a neutron star crust}},
url = {http://stacks.iop.org/0954-3899/42/i=10/a=105201?key=crossref.01f2cf68c4b668883706242ad0248b44},
volume = {42},
year = {2015}
}
@article{Burvenich2007,
abstract = {The properties of nuclei embedded in an electron gas are studied within the relativistic mean-field approach. These studies are relevant for nuclear properties in astrophysical environments such as neutron-star crusts and supernova explosions. The electron gas is treated as a constant background in the Wigner-Seitz cell approximation. We investigate the stability of nuclei with respect to $\alpha$ and $\beta$ decay. Furthermore, the influence of the electronic background on spontaneous fission of heavy and superheavy nuclei is analyzed. We find that the presence of the electrons leads to stabilizing effects for both $\alpha$ decay and spontaneous fission at high electron densities. Furthermore, the screening effect shifts the proton dripline to more proton-rich nuclei, and the stability line with respect to $\beta$-decay is shifted to more neutron-rich nuclei. Implications for the creation and survival of very heavy nuclear systems are discussed.},
archivePrefix = {arXiv},
arxivId = {arXiv:0706.1450v1},
author = {B{\"{u}}rvenich, Thomas J. and Mishustin, Igor N. and Greiner, Walter},
doi = {10.1103/PhysRevC.76.034310},
eprint = {arXiv:0706.1450v1},
issn = {05562813},
journal = {Physical Review C - Nuclear Physics},
number = {3},
title = {{Nuclei embedded in an electron gas}},
volume = {76},
year = {2007}
}

